AUTONAV: A Toolfor Autonomous Navigation of Robots

We present a tool AUTONAV that automates the mapping, localization, and path-planning tasks for autonomous navigation of robots. The modular architecture allows easy integration of various algorithms for these tasks for comparison. We present the generated maps and path-plans by AUTONAV in indoor simulation scenarios.

==> abstract.tex <==
\begin{abstract}
\begin{comment}
With the resent advancement in the field of robotics, it opens a growing interest to use automated robots in many application areas of every day life. Navigation of these automated robots has become a topic of huge importance as many applications require the robots to move with in a constricted scenario.

However, navigation in robotics is always a very challenging task as it takes different complex sub tasks to act together smoothly and error-freely to make navigation possible. The primary sub tasks that builds a navigation system for a robot comprises of designing the motion primitives for the robot, recognizing the environment in which it operates and motion-planning which itself consists of two sub-tasks: path-planning and robot controller. While path-planning is to find a feasible path from a source location to a destination, the controller guides the robot along the path to reach  the destination. As all of these tasks go through several trial-and-errors and reconciliations phases before having a reasonably accurate navigation system for a robot. Therefore, before implementing in the real world it is better to test these capabilities in the simulation environment which can prevent much hardware damages that may happen otherwise.

In this paper we have gone through all of these sub tasks of a navigation system in details from designing the motion primitives for a robotic Lizard to generating map of the environment to motion-planning. Path-planning is the major concern of this paper, where we pose the path-planning problem as a constraint satisfaction problem. The path-planning constraints are represented as SMT-encoded first-order logic formulae and solve by a state-of the-art SMT solver. All the experiments are done in CoppeliaSim\cite{coppeliaSim} simulation environment.
\end{comment}

We present \textsc{Autonav} that automates the mapping, localization and path-planning tasks for autonomous navigation of robots. The modular architecture allows easy integration of various algorithms for these tasks for a comparison. We present the generated maps and path-plans by \textsc{Autonav} in indoor simulation scenarios.
% We further divided the motion planning problem into two sub-tasks: path-planning and robot controller.
%Motion-planning problem remained the main focus of this paper and represented as SMT-constraint satisfaction problem and solve by a state-of the-art SMT solver\cite{10.1007/978-3-540-78800-3_24}.
% A robot controller line-of-sight(Los) algorithm is also devised to guide the robot along a path.
%All the experiments are done in CoppeliaSim\cite{coppeliaSim} simulation environment integrated with ROS.
\end{abstract}

==> cartographer-map.tex <==
\section{2D Map generation using Cartographer}
\begin{wrapfigure}{r}{0.5\textwidth}
     \vspace{-20pt}
     \centering
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/sim_env.png}
         \caption{Environment}
         \label{fig:sim_env}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/map5.png}
         \caption{2D map}
         \label{fig:map}
     \end{subfigure}
  %\vspace{-10pt}
  \caption{Environment and 2D map.}
  \vspace{-20pt}
  \label{fig:env_map}
\end{wrapfigure}

We have built 2d mapping using the \emph{Cartographer}\cite{45466} tool that provides real-time simultaneous localization and mapping (SLAM) in 2D and 3D across multiple platforms and sensor configurations, encoding information about obstacles, free spaces and unknown regions of the simulation environment as occupancy grid map in ROS environment while taking in lidar sensor and odometry data from the robot. The CoppeliaSim simulation environment has a dimension of $10m\times10m$ surrounded by walls (see in Figure \ref{fig:env_map}(a)). The 2d map that we generated in accordance with our environment is extended by $0.5m$ of additional spaces in each side (see in Figure \ref{fig:env_map}(b)).
% \begin{figure}[htbp]
 %   \centering
 %   \includegraphics[width=0.5\textwidth]{Images/map5.png}
 %   \caption{2D Map}
 %  \label{fig:map}
% \end{figure}
\begin{comment}
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.25\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/sim_env.png}
         \caption{Simulation environment}
         \label{fig:sim_env}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.2\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/map5.png}
         \caption{2D map}
         \label{fig:map}
     \end{subfigure}
        \caption{Simulation environment and 2D map.}
        \label{fig:env_map}
\end{figure}
\end{comment} 


==> motion-planning.tex <==
\section{Motion Planning}
In this section, we first describe the design of our \emph{Lizard-bot} in the following text. Then, we illustrate the set of \emph{motion primitives} that could be actuated in our robot. A motion-plan will consist of composition of these primitives applied at distinct points in time along a path.

\textbf{Robot Configuration:} \emph{Lizard-Bot} has \emph{front-link} and \emph{back-link} attached with the \emph{base-link}. These \emph{front-link} and \emph{back-link} can rotate upto $45\degree$ w.r.t \emph{base-link}. Two legs that can be lifted or grounded are attached with \emph{front-link} and \emph{back-link} each.


%Atul, Satyendra to write on the robot hardware description briefly
\subsection{Robot Motion Primitives}
Motion primitives are a set of control actions that can be provided as commands to our robot for execution. 
%We now present four basic primitives, \emph{move-forward}, \emph{move-backward}, \emph{rotate-clockwise} and \emph{rotate anti-clockwise} and the principles behind the implementation of the primitives. The rotational movements \emph{rotate-clockwise} and \emph{rotate anti-clockwise}, each has four discretizations ($6{\degree}$, $4.5{\degree}$, $3{\degree}$ and $1.5{\degree}$). 
%Thus, our robot's ten degrees-of-freedom comprises two linear movements (\emph{move-forward} and \emph{move-backward}) and eight rotational movements (four discrete \emph{rotate-clockwise} and \emph{rotate anti-clockwise} rotations each). %We begin with the definition of a state of a robot.
Our robot has four basic primitives, \emph{move-forward} and \emph{move-backward} is for linear movements and \emph{rotate-clockwise} and \emph{rotate anti-clockwise} is for rotational movements (each rotational movement has four discretizations $6{\degree}$, $4.5{\degree}$, $3{\degree}$ and $1.5{\degree}$) which constitutes robot's ten degrees-of-freedom.

%\begin{definition}The state of a robot at a time instant $t$ denoted as $R(t)$ is a three-tuple ($R_x$,$R_y$,$R_{\theta}$), where $R_x$, $R_y$ are the $x$ and $y$ coordinates of the robot and $\theta$ is the orientation of the robot with respect to a fixed frame of reference.
%\end{definition}

%Sajid: Introduce the motion primitives/actions
Each of the motion primitives has two phases, and when applied on the \emph{Lizard-Bot} will perform a complete movement such as a linear forward or backward movement or a rotational clockwise or anti-clockwise movement. A description of these motion primitives for the forward and one discretization ($6{\degree}$) of the clockwise rotational movement are given as reference.
%A detailed description of these motion primitives for the forward and backward movement and one discretization ($6{\degree}$) of the rotational clockwise and anti-clockwise movement are given below:
\begin{enumerate}


% Move forward: Describe how does the robot move a step forward. what is the minimum distance that could be traversed forward on the application of one move-forward primitive/action?
    \item {\textbf{Move-forward:} The motion primitive \emph{move-forward} is used to perform one complete forward movement for the \emph{Lizard-Bot}.
    
    
    In the first phase, the \emph{Lizard-Bot} lifts its front-right and back-left legs together while front-joint and back-joint are rotated with $30{\degree}$ and $-30\degree$ angle respectively. As front-left and back-right legs are grounded at that time, the rotations of front-joint and back-joint make the front-right and back-left legs get forwarded (see Figure \ref{fig:lizard-bot_movement}(a)first phase where $\theta_f = -\theta_b = 30\degree$).
    
    
    In the second phase, the \emph{Lizard-Bot} lifts its front-left and back-right legs together while front-joint and back-joint are rotated with $-30\degree$ and $30\degree$ angle respectively (see Figure \ref{fig:lizard-bot_movement}(a)second phase where $-\theta_f = \theta_b = 30\degree$). This time these two legs get forwarded and thus completes one forward movement.
    
    As a result of one such complete forward movement the effective displacement of the \emph{Lizard-Bot} is $6.46$ cm (the effective displacement of the robot is calculated from \textit{CoppeliaSim} simulation environment).
    %\begin{figure}[htbp]
     %   \centering
       % \includegraphics[width=0.5\textwidth]{Images/Lizard_fwd_move.png}
        %\caption{Lizard-Bot forward movement}
        %\label{fig:fwd_move}
    %\end{figure}
    }

% Move backward: Describe how does the robot move a step backward. what is the minimum distance that could be traversed backward on the application of one move-backward primitive/action?
    %\item {\textbf{Move-backward:} The motion primitive \emph{move-backward} will cause one complete movement in the backward direction for our \emph{Lizard-Bot}.
    
    %The action sequences of \emph{move-backward} primitive is just opposite of \emph{move-forward}. Here, the first phase comprises of lifting front-right and back-left legs of \emph{Lizard-Bot} together and rotating front-joint and back-joint with $-30\degree$ and $30\degree$ angle respectively, while in the second phase front-left and back-right legs are lifted together and front-joint and back-joint are rotated with $30{\degree}$ and $-30\degree$ angle respectively. The effective displacement for one complete backward movement of the \emph{Lizard-Bot} is $6.46$ cm.
    %}
 % Rotate clockwise (RotClk): Describe how does the robot rotate clockwise. what is the minimum angle that the robot could rotate in the clockwise direction on the application of one RotClk primitive/action? 
    \item {\textbf{Rotate clockwise (RotClk):} The motion primitive that will cause the \emph{Lizard-Bot} to make a clockwise angular rotation (right turn) is \emph{RotClk}.
    
    In the first phase, \emph{Lizard-Bot} lifts its front-left and back-right legs together while front-joint and back-joint are rotated with $\theta_f$ and $\theta_b$ respectively (see Figure \ref{fig:lizard-bot_movement}(b)first phase where $-\theta_f = \theta_b = 45\degree$). In the second phase, \emph{Lizard-Bot} lifts its front-right and back-left legs together while front-joint and back-joint are rotated with $20\degree$ and $-20\degree$ angle respectively (see Figure \ref{fig:lizard-bot_movement}(b)second phase where $\theta_f = -\theta_b = 20\degree$).
    
    One such complete \emph{RotClk} movement (right turn) will rotate \emph{Lizard-Bot} clockwise a certain angle $\alpha$ which is effective angular rotation. This $\alpha$ depends on the angle $\gamma$, given as:
    %\begin{equation}\scriptsize
     %   \gamma = K * \alpha
    %\end{equation}
    {\scriptsize \[\gamma = K * \alpha\]}
    where $\gamma = \|\theta_1\|-\|\theta_2\|$, $\theta_1$ and $\theta_2$ are angle of rotation of front-joint and back-joint in the first and second phase respectively while K is known as proportional gain and have to tune its value by multiple trials. In this case, $\|\alpha\|=6\degree$ as $\gamma=25\degree$.
    }
    %\begin{figure}[htbp]
     %   \centering
      %  \includegraphics[width=0.8\textwidth]{Images/Lizard_right_turn.png}
       % \caption{Lizard-Bot RotClk movement (right turn)}
        %\label{fig:right_turn}
    %\end{figure}
    \begin{figure}[htbp]
      \vspace{-20pt}
      \centering
      \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/Lizard_fwd_move.png}
         \caption{Lizard-Bot forward movement}
         \label{fig:fwd_movement}
      \end{subfigure}
      \hfill
      \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{Images/Lizard_right_turn.png}
         \caption{Lizard-Bot RotClk movement}
         \label{fig:right_turn}
      \end{subfigure}
      \caption{Lizard-Bot movement.}
      \label{fig:lizard-bot_movement}
      \vspace{-20pt}
    \end{figure}   
% Rotate anticlockwise (RotAclk): describe how does the robot rotate anticlockwise. What is the minumum angle that the robot could roate in the anticlockwise direction, upon the application of one RotAclk primitive/action?
    %\item {\textbf{Rotate anti-clockwise (RotAclk):} The motion primitive \emph{RotAclk} will enable \emph{Lizard-Bot} to perform anti-clockwise angular movement (left turn).
    
    %The action sequences for \emph{RotAclk} is similar to \emph{RotClk} but opposite. In this case, the front-right and back-left legs of \emph{Lizard-Bot} will be lifted together then front-joint and back-joint will be rotated with $45\degree$ and $-45\degree$ angle respectively in the first phase, while in the second phase front-left and back-right legs will be lifted together followed by $-20\degree$ and $20\degree$ rotation of the front-joint and back-joint respectively. The effective angular rotation is $\|\alpha\|=6\degree$ for \emph{RotAclk} also.
    %}
% Can we make the robot accelerate? 
\end{enumerate}

%\begin{table}[]
\begin{wraptable}{r}{0.5\textwidth}
    \vspace{-20pt}
    \scriptsize
    \centering
    \begin{tabular}{|c|c|c|c|c|}
    \hline
         \multicolumn{1}{|p{1.3cm}|}{\centering Rot \\ $\|\theta_1\|$, $\|\theta_2\|$}
         & \multicolumn{1}{|p{1.2cm}|}{\centering Rot diff \\ ($\lambda$)} & \multicolumn{1}{|p{1.3cm}|}{\centering Eff rot \\ ($\theta$)} 
         & \multicolumn{1}{|p{1.2cm}|}{\centering Ratio \\ ($K$)}\\
    \hline
         $45{\degree}$ , $20{\degree}$ & $25{\degree}$ & $5.947{\degree}$ & $4.204$\\
         $40{\degree}$ , $20{\degree}$ & $20{\degree}$ & $4.535{\degree}$ & $4.414$\\
         $35{\degree}$ , $20{\degree}$ & $15{\degree}$ & $3.072{\degree}$ & $4.883$\\
         $30{\degree}$ , $20{\degree}$ & $10{\degree}$ & $1.485{\degree}$ & $6.734$\\
         $30{\degree}$ , $30{\degree}$ & $0{\degree}$ & $0{\degree}$ & $-$\\
    \hline 
    \end{tabular}
    \caption{Clockwise and anti-clockwise rotations.}
    \vspace{-20pt}
    \label{tab:table1}
\end{wraptable}
%\end{table}
In table \ref{tab:table1}, we have shown different discretization of clockwise and anti-clockwise rotational movement of the \emph{Lizard-Bot} achieving through by applying different $\theta_1$ and $\theta_2$ rotation to the joints in both phases of movement where \emph{Rot diff} is rotational difference in both phases, \emph{Eff rot} is effective rotation of the robot and $Ratio\ K$ is the ratio of $\lambda/\theta$.

%\subsubsection{State Transitions on Application of Motion Primitives} Application of the above motion primitives update the state of the robot R(t). We provide the state-transition relation for each of the primitive.

\subsection{Path Planning as Constraint Satisfaction Problem}
To represent the path-planning problem as a constraint satisfaction problem, we encoded the above motion primitives of our \emph{Lizard-Bot} along with the initial and goal condition and constraints from the map as SMT-encoded first-order logic formulae.

Let, $x_t$ and $y_t$ are two variables that represents robot's position and $\theta_t$ represents robot's orientation w.r.t $+ve$ $X$-$axis$ in the map at time instance $t$ where $0\leq t\leq M$, where as $v_x$ and $v_y$ are the velocities of the robot in $X$ and $Y$ directions respectively.
\begin{definition}
An \textbf{initial state} is a pair $\langle Init, I\_cnstr \rangle$ where $Init$ is a tuple $\langle x_{init}, y_{init}, \theta_{init}\rangle$, where $(x_{init}, y_{init}) \in \mathbb{R}^2$  and $\theta_{init} \in\ [0, 2\pi]$ defines the initial position and orientation of the robot and $I\_cnstr$ is a set of constraints that represent the environment in the map. The initial state is encoded in SMT as below:
%\begin{equation}\scriptsize
  %Init: (x_0=x_{init})\land(y_0=y_{init})\land(\theta_0=\theta_{init})
%\end{equation}
%\begin{equation}\scriptsize
%  I\_cnstr: \forall t\in [0, M], (x_t\neq x_{obs})\land(y_t\neq y_{obs}) 
%\end{equation}
{\scriptsize
\[Init: (x_0=x_{init})\land(y_0=y_{init})\land(\theta_0=\theta_{init})\]
\[I\_cnstr: \forall t\in [0, M], (x_t\neq x_{obs})\land(y_t\neq y_{obs})\]}
where $(x_{obs},y_{obs}) \in OBS$, $OBS$ is the set of obstacles in the map.
\end{definition}

\begin{definition}
A \textbf{goal state} is a pair $\langle Goal, G\_cnstr \rangle$ where $Goal$ is a tuple $\langle x_g, y_g, \theta_g\rangle$, where $(x_g, y_g) \in \mathbb{R}^2$  and $\theta_g \in\ [0, 2\pi]$ defines the goal position and orientation of the robot and $G\_cnstr$ is a set of additional goal constraints such as, if $(x_t, y_t)$ and $(x_{t+1}, y_{t+1})$ two consecutive way-points in robot's path, then a line between them does not intersect with any obstacle OBS.

The goal state is encoded as below:
%\begin{equation}\scriptsize
 % Goal: \bigvee_{1\leq t\leq M} [(x_t=x_g)\land(y_t=y_g)\land(\theta_t=\theta_g)]
%\end{equation}
%\begin{equation}\scriptsize
 % G\_cnstr: \forall t\in [0, M], \{\|x,y\|\}\notin OBS\ satisfies\ y = \frac{(y_{t+1}-y_t)} {(x_{t+1}-x_t)} * x + c) 
%\end{equation}
{\scriptsize
\[Goal: \bigvee_{1\leq t\leq M} [(x_t=x_g)\land(y_t=y_g)\land(\theta_t=\theta_g)]\]
\[G\_cnstr: \forall t\in [0, M], \{\|x,y\|\}\notin OBS\ satisfies\ y = \frac{(y_{t+1}-y_t)} {(x_{t+1}-x_t)} * x + c)\]
}
\end{definition}
The motion-primitives that we have formulated are used to facilitate the movement for our \emph{Lizard-Bot} in the scenario.
\begin{definition}
The movement \textbf{mov} can be defined as a pair $\langle R(t), R(t+1)\rangle$ where $R(t)$ and $R(t+1)$ are states of the robot at time instance $t$ and $t+1$ respectively. An application of a motion-primitive $p\in P$ ($P$ is the set of all motion-primitives) at time $t$ derives $R(t+1)$ form $R(t)$.

The movement is encoded as below:
\begin{equation} \label{eq1}\scriptsize
\begin{split}
Mov:\bigwedge_{0\leq t<M} &\bigg [[(x_{t+1}=x_t + v_x*\cos\theta)\land(y_{t+1}=y_t + v_y*\sin\theta)\land(\theta_{t+1}=\theta_t)] \\
 & \lor [(x_{t+1}=x_t - v_x*\cos\theta)\land(y_{t+1}=y_t - v_y*\sin\theta)\land(\theta_{t+1}=\theta_t)] \\
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t + 6)]  \\
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t + 4.5)] \\ 
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t + 3)] \\ 
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t + 1.5)] \\ 
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t - 6)] \\
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t - 4.5)] \\ 
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t - 3)] \\ 
 & \lor [(x_{t+1}=x_t)\land(y_{t+1}=y_t)\land(\theta_{t+1}=\theta_t - 1.5)] \bigg ] \\ 
\end{split}
\end{equation}
\end{definition}
%\begin{definition}
To optimise the feasible path, we construct a new constraint that ensure that the robot takes minimum number of turns to reach the goal position and avoiding the unnecessary turn.
%\end{definition}
%In Figure \ref{fig:result}, Result 1 represents a feasible path from initial to goal positions before optimization and the Result 2 represents a feasible path after applying the optimization constraint,considering the initial and goal position are same in the both images.
%\\For implementing this constraints, we consider m number of variables $M_t$ $\forall t \in \{0,1,2...m-2\}$ ( m is the number of time instances required to reach the goal position) and a checking condition that if the positions of the robot are collinear in between three consecutive time step $t$ , $t+1$ , $t+2$ then we add 1 to $M_t$ variable and then we maximize the summation $\Sigma M_t$, $\forall t \in \{0,1,2....m-2\}$
%    \vspace{0.1cm}
The constraint is encoded as below:
%    \vspace{0.1cm}
    \\ if ($( x_t$ - $x_{t+1} )$ = $( x_{t+1}$ - $ x_{t+2} ) $ and $( y_t$ - $y_{t+1} )$ = $( y_{t+1}$ - $y_{t+2} ) $) 
    \\then $M_t = 1$ , else  $M_t = 0$
%    \vspace{0.15cm}
    \\maximize ($\Sigma M_t$)\hspace{0.5cm}     where $\forall t \in \{0,1....m\}$.





==> navigation.tex <==
\section{Robot Controller} %Navigation for Lizard-bot
We have designed a robot controller for line-of-sight navigation for our \emph{Lizard-Bot} to control the movement along the path given by the SMT solver to reach a destination. The detail of the \emph{LoS algorithm} is as follows:

%\subsection{Line of Sight(LoS) algorithm}
\textbf{Line of Sight(LoS) algorithm:} The \emph{LoS algorithm} works in three steps. a) Calculate the effective angle: takes the co-ordinates of the next way-point from the suggested path and calculated the angle at which it situates from robot's current position and orientation. b) Rotation: then rotate the robot towards goal accordingly. Each rotational movement is followed by a backward movement to minimize the positional changes during rotation is due to unavailability of in-place rotation for our \emph{Lizard-Bot}. c) Move: finally calculate the distance and number of steps needed to reach the goal and move accordingly. Our \emph{LoS algorithm} can quite accurately helps the robot to reach a given goal position in the simulated environment.

%\begin{wrapfigure}{l}{0.5\textwidth}
%\vspace{-20pt}
%\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
  \scriptsize
  \caption{LoS algorithm}
  \LinesNumbered
  \SetAlgoLined
  \Begin{
    \KwIn{Take $(x,y)$ co-ordinates of the goal position\\}
     Let, $(x_R, y_R)$ and $\theta_R$ be robot's current co-ordinates and orientation with $X-axis$.\\
     Calculate the angle $\phi$ between the robot's current position $(x_R,y_R)$ and goal position $(x,y)$ w.r.t +ve $X-axis$
     Calculate the effective angle, $\theta \gets \phi-\theta_R$\\
     \If{$\theta > 180$}{$\theta \gets \theta - 360$}
     Rotate clockwise or anti-clockwise to cover the angle $\theta$
     \tcp*{Each rotational movement is followed by a move backward movement}
     Calculate the distance $dist \gets \sqrt{(x-x_R)^2 + (y-y_R)^2}$\\
     Calculate the $n\_steps \gets dist/6.46$
    \tcp*{The number of linear movements needed to cover the distance}
    Move-forward to cover the distance.
  }
\end{algorithm}
%\end{minipage}
%\vspace{-20pt}
%\end{wrapfigure}

\begin{comment}

\begin{wrapfigure}{l}{0.5\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\scriptsize
\caption{LoS algorithm : (a) calculate the effective angle}
\LinesNumbered
\SetAlgoLined
\Begin{
\KwIn{Take $(x,y)$ co-ordinates of the goal position\\}
 Let, $(x_R, y_R)$ and $\theta_R$ be robot's current co-ordinates and orientation with $X-axis$.\\
 \tcc{Calculate the angle between current and goal position}
 \If{$(x-x_R)>0\ \land\ (y-y_R)>0$}{$\phi \gets \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \ElseIf{$((x-x_R)<0\ \land\ (y-y_R)>0))\ \lor\ ((x-x_R)<0\ \land\ (y-y_R)<0)$}{$\phi \gets 180 + \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \ElseIf{$(x-x_R)>0\ \land\ (y-y_R)<0)$}{$\phi \gets 360 + \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \tcc{Calculate the effective angle $\theta$}
 $\theta \gets \phi-\theta_R$\\
 \If{$\theta > 180$}{$\theta \gets \theta - 360$}
 }
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
\scriptsize
\caption{LoS algorithm : (b) rotate clockwise or anti-clockwise}
%\begin{multicols}{2}
\LinesNumbered
\SetAlgoLined
 \Begin{
 \KwIn{Effective angle $\theta$\\}
 \tcc{Rotate clockwise or anti-clockwise to cover the angle $\theta$}
 \While{$\theta \geq 1.5\ \lor\ \theta \leq -1.5$}{
    \If{$\theta \geq 6$}{
    \emph{RotClk\_6}\\
    $\theta \gets \theta-6$}
    \ElseIf{$\theta \geq 4.5\ \land\ \theta<6$}{
    \emph{RotClk\_4.5}\\
    $\theta \gets \theta-4.5$}
    \ElseIf{$\theta \geq 3\ \land\ \theta<4.5$}{
    \emph{RotClk\_3}\\
    $\theta \gets \theta-3$}
    \ElseIf{$\theta \geq 1.5\ \land\ \theta<3$}{
    \emph{RotClk\_1.5}\\
    $\theta \gets \theta-1.5$}
    \ElseIf{$\theta \leq -1.5\ \land\ \theta>-3$}{
    \emph{RotAclk\_1.5}\\
    $\theta \gets \theta+1.5$}
    \ElseIf{$\theta \leq -3\ \land\ \theta>-4.5$}{
    \emph{RotAclk\_3}\\
    $\theta \gets \theta+3$}
    \ElseIf{$\theta \leq -4.5\ \land\ \theta>-6$}{
    \emph{RotAclk\_4.5}\\
    $\theta \gets \theta+4.5$}
    \ElseIf{$\theta \leq -6$}{
    \emph{RotAclk\_6}\\
    $\theta \gets \theta+6$}
    \emph{Move-backward}
 }
 }
%\end{multicols}
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\begin{wrapfigure}{r}{0.5\textwidth}
\begin{minipage}{0.45\textwidth}
\begin{algorithm}[H]
  %\algsetup{linenosize=\tiny}
  \scriptsize
  \caption{LoS algorithm : (a) move}
  \LinesNumbered
  \SetAlgoLined
  \Begin{
    \KwIn{Take $(x,y)$ co-ordinates of the goal position\\}
    \tcc{Calculate the distance $dist$ of the goal position}
    $dist \gets \sqrt{(x-x_R)^2 + (y-y_R)^2}$\\
    $n\_steps \gets dist/6.46$ \tcp*{The number of linear movements needed to cover the distance}
    \For{$i \gets 1$ \textbf{to} $n\_steps$}{
          \emph{Move-forward}\;
    }
  }
\end{algorithm}
\end{minipage}
\end{wrapfigure}

\end{comment}

\begin{comment}
\begin{algorithm}[H]
\caption{LoS algorithm}
\LinesNumbered
\SetKwBlock{Begin}{Begin}{}
\SetAlgoLined
%\KwResult{Write here the result }
%\begin{algorithmic}
 \Begin{
 \KwIn{Take $(x,y)$ co-ordinates of the goal position\\}
 Let, $(x_R, y_R)$ and $\theta_R$ be robot's current co-ordinates and orientation with $X-axis$.\\
 \tcc{Calculate the angle between current and goal position}
 \If{$(x-x_R)>0\ \land\ (y-y_R)>0$}{$\phi \gets \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \ElseIf{$((x-x_R)<0\ \land\ (y-y_R)>0))\ \lor\ ((x-x_R)<0\ \land\ (y-y_R)<0)$}{$\phi \gets 180 + \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \ElseIf{$(x-x_R)>0\ \land\ (y-y_R)<0)$}{$\phi \gets 360 + \tan^{-1}{\frac {(y-y_R)} {(x-x_R)}}$}
 \tcc{Calculate the effective angle $\theta$}
 $\theta \gets \phi-\theta_R$\\
 \If{$\theta > 180$}{$\theta \gets \theta - 360$}
 }            \tcp*{cont. next page}
\end{algorithm}

\SetNlSty{texttt}{(}{)}
\begin{algorithm}
  \LinesNumbered
\setcounter{AlgoLine}{15}
% This is to restore vline mode if you did not take the package as \usepackage[linesnumbered,ruled,vlined]{algorithm2e}
  \SetAlgoVlined
%This is to hide Begin keyword
\SetKwBlock{Begin}{}{end}
 \Begin{
 \tcc{Rotate clockwise or anti-clockwise to cover the angle $\theta$}
 \While{$\theta \geq 1.5\ \lor\ \theta \leq -1.5$}{
    \If{$\theta \geq 6$}{
    \emph{RotClk\_6}\\
    $\theta \gets \theta-6$}
    \ElseIf{$\theta \geq 4.5\ \land\ \theta<6$}{
    \emph{RotClk\_4.5}\\
    $\theta \gets \theta-4.5$}
    \ElseIf{$\theta \geq 3\ \land\ \theta<4.5$}{
    \emph{RotClk\_3}\\
    $\theta \gets \theta-3$}
    \ElseIf{$\theta \geq 1.5\ \land\ \theta<3$}{
    \emph{RotClk\_1.5}\\
    $\theta \gets \theta-1.5$}
    \ElseIf{$\theta \leq -1.5\ \land\ \theta>-3$}{
    \emph{RotAclk\_1.5}\\
    $\theta \gets \theta+1.5$}
    \ElseIf{$\theta \leq -3\ \land\ \theta>-4.5$}{
    \emph{RotAclk\_3}\\
    $\theta \gets \theta+3$}
    \ElseIf{$\theta \leq -4.5\ \land\ \theta>-6$}{
    \emph{RotAclk\_4.5}\\
    $\theta \gets \theta+4.5$}
    \ElseIf{$\theta \leq -6$}{
    \emph{RotAclk\_6}\\
    $\theta \gets \theta+6$}
    \emph{Move-backward}
 }
 \tcc{Calculate the distance $dist$ of the goal position}
 $dist \gets \sqrt{(x-x_R)^2 + (y-y_R)^2}$\\
 $n\_steps \gets dist/6.46$ \tcp*{The number of linear movements needed to cover the distance}
 \For{$i \gets 1$ \textbf{to} $n\_steps$}{
  \emph{Move-forward}\;
 }
 }
%\end{algorithmic}
%\caption{LoS algorithm}
\end{algorithm}
\end{comment}

%\subsection{Lizard-Bot visiting few way-points using LoS navigation}


==> preliminaries.tex <==
\section{Preliminaries}

